Temporal Answer Set Programming on Finite Traces

In this paper, we introduce an alternative approach to Temporal Answer Set Programming that relies on a variation of Temporal Equilibrium Logic (TEL) for finite traces. This approach allows us to even out the expressiveness of TEL over infinite traces with the computational capacity of (incremental) Answer Set Programming (ASP). Also, we argue that finite traces are more natural when reasoning about action and change. As a result, our approach is readily implementable via multi-shot ASP systems and benefits from an extension of ASP's full-fledged input language with temporal operators. This includes future as well as past operators whose combination offers a rich temporal modeling language. For computation, we identify the class of temporal logic programs and prove that it constitutes a normal form for our approach. Finally, we outline two implementations, a generic one and an extension of clingo.

==> motivation.tex <==
\section{Motivation}

To motivate our goals, let us consider the following simplification of the Yale Shooting Scenario where shooting a loaded gun just unloads the gun, if there is not any abnormal failure.
A typical encoding of this scenario in ASP could look like:
\begin{eqnarray}
\loaded(T) & \leftarrow & \load(T), T>0 \label{f:ys1}\\
\bot & \leftarrow & \load(T), \loaded(\prT), T>0 \label{f:ys2}\\
\unloaded(T) & \leftarrow & \shoot(T), \loaded(\prT), T>0, \Not \fail(T) \label{f:ys3}\\
\loaded(T) & \leftarrow & \loaded(\prT), T>0, \Not \unloaded(T) \label{f:ys4}\\
\unloaded(T) & \leftarrow & \unloaded(\prT), T>0, \Not loaded(T) \label{f:ys5}\\
\shoot(T) \vee \load(T) \vee \wait(T) & \leftarrow & T>0\label{f:ys6}
\end{eqnarray}
\begin{lstlisting}[basicstyle=\ttfamily\small]
  loaded(T) :- load(T), T>0.
            :- load(T), loaded(T-1), T>0.
unloaded(T) :- shoot(T), loaded(T-1), T>0, not fail(T).
  loaded(T) :-   loaded(T-1), T>0, not unloaded(T).
unloaded(T) :- unloaded(T-1), T>0, not loaded(T).
shoot(T) ; load(T) ; wait(T)  :-  T>0.
\end{lstlisting}

where $T$ is some integer variable we would ground for values $T=0..n$ for some finite horizon $n \geq 0$.
Rules \eqref{f:ys1} and \eqref{f:ys2} respectively describe the effect and the precondition of action $\load$.
Rule \eqref{f:ys3} describes the effects of shooting a loaded gun (that does not fail).
We assume we can always shoot, even if the gun is unloaded.
\eqref{f:ys4} and \eqref{f:ys5} are the inertia default for fluents $\loaded/\unloaded$.
Finally, \eqref{f:ys6} is used to generate an action for each  state $T>0$.
As a quite trivial planning problem, imagine we want to find a way to unload a gun.
To do so, we would add the rules
\begin{eqnarray}
\unloaded(0) & & \label{f:ys10}\\
\bot & \leftarrow & \Not goal(n) \label{f:ys12}\\
goal(T) & \leftarrow & \unloaded(T), \loaded(\prT), T>0 \label{f:ys13}
\end{eqnarray}
\begin{lstlisting}[basicstyle=\ttfamily\small]
unloaded(0).
  :-  not goal(n)
goal(T) :- unloaded(T), loaded(T-1), T>0
\end{lstlisting}
to force plans that end up at the moment a loaded gun is unloaded.
Let us call $\Pi$ to the resulting program.
If we ground $\Pi$ for $T=1$, no solution is found, but for $T=2$ we get one answer set that includes the sequence of actions $\load(1)$ and $\shoot(2)$, being the shortest solution to our planning problem.
If we keep increasing $T$, new plans are obtained that introduce irrelevant steps (inserting $\wait$ actions) but are still correct solutions.
In fact, there is a one-to-one correspondence between each answer set of $\Pi$ and a solution to our planning problem (a finite sequence of actions that ends unloading the gun).

Now, consider the encoding of this problem in Temporal Equilibrium Logic.
The formulation is more or less straightforward:
\begin{eqnarray}
\Next \alwaysF (\load & \to & \loaded) \label{f:ys1b}\\
\Next \alwaysF (\load \wedge \previous \loaded & \to & \bot) \label{f:ys2b}\\
\Next \alwaysF (\shoot \wedge \previous \loaded \wedge \neg \fail & \to & \unloaded) \label{f:ys3b}\\
\Next \alwaysF (\previous \loaded \wedge \neg \unloaded & \to & \loaded) \label{f:ys4b}\\
\Next \alwaysF (\previous \unloaded \wedge \neg \loaded & \to & \unloaded) \label{f:ys5b}\\
& & \Next \alwaysF (\shoot \vee \load \vee \wait) \label{f:ys6b}
\end{eqnarray}
where \eqref{f:ys1b}-\eqref{f:ys6b} respectively correspond to \eqref{f:ys1}-\eqref{f:ys6}.
The initial situation would just be defined by the formula $\unloaded$ whereas \eqref{f:ys12} becomes the formula $\neg \eventuallyF goal \to \bot$, that can be read as ``avoid traces where $goal$ is never reached,'' while \eqref{f:ys13} would become $\Next \alwaysF (\unloaded \wedge \previous \loaded \to goal)$.
It is important to note a substantial difference with respect to the ASP program.
Temporal stable models in \TEL{} always have the form of infinite traces.
As a result, the shortest solution we found before (loading and the shooting) will be now included as the prefix of an infinite number of infinite plans where, after the goal has been reached, we go on performing irrelevant actions forever, like waiting, or loading and shooting the gun even though we already reached the goal before.
For instance, one of those cases is given by the regular expression $\load \ \shoot \ \wait\ ^\omega$.
It is clear, thus, that we lose the one-to-one correspondence between each temporal stable model and each possible solution to the planning problem, since in order to obtain a \emph{finite plan}, we must extract the finite prefix from each infinite temporal stable model, stopping at the point where $goal$ becomes true for the first time.

{\color{blue} Apart from the adequacy of dealing with finite traces, another interesting issue has to do with the use of temporal operators.
As we saw, in the temporal representation, operators are directed to the future, using `$\Next$' to represent the successor state, whereas in the ASP program, the successor state $T$ is the ``present'' and the previous one $\prT$ is ``in the past.''
This is more intuitive in the sense that, in this way, the ground program for $\prT$ constitutes a piece of representation completely independent from the one for $T$.}
Moreover, we claim that, when using causal reading of program rules, it is generally more interesting to refer to the past information in the rule body and use future time operators for information to be derived in the rule head.
Consider, for instance, the following specification {\em ``If we make two shots while the gun was never loaded, then some failure will eventually occur.''}
This piece of knowledge could be captured by a rule like:
\begin{eqnarray}
\alwaysF (\eventuallyF \fail & \leftarrow & \shoot \wedge \alwaysP \unloaded \wedge \previous \eventuallyP \shoot) \label{f:fail}
\end{eqnarray}
If, for instance, we want to generate a trace that explains why shooting a loaded gun does not unload the gun, we could include the goal:
\begin{eqnarray*}
goal & \leftarrow & \shoot \wedge \previous \loaded \wedge \loaded
\end{eqnarray*}
to obtain the shortest explanation $\langle \shoot,\shoot,\load,\shoot \rangle$ where the gun happens to fail precisely at the last situation.

Of course, in order to capture this behavior in ASP, we could use auxiliary predicates to keep track of the trace history or to force $\fail$ to become true in the future as follows:
\begin{eqnarray*}
\text{\em willfail}(T) \vee \fail(T) & \leftarrow & \shoot(T), \Not \text{\em loadedonce}(T), \text{\em shotonce}(\prT) \\ 
\text{\em loadedonce}(T) & \leftarrow & \loaded(T) \\
\text{\em loadedonce}(T) & \leftarrow & \text{\em loadedonce}(\prT)\\
\text{\em shotonce}(T) & \leftarrow & \shoot(T) \\
\text{\em shotonce}(T) & \leftarrow & \text{\em shotonce}(\prT)\\
\text{\em willfail}(T) \vee \fail(T) & \leftarrow & \text{\em willfail}(\prT), \Not \fail(\prT)\\
\fail(n) & \leftarrow & \text{\em willfail}(n)
\end{eqnarray*}
but this is obviously less succint and more prone to errors than \eqref{f:fail}.

In the next section we proceed to provide an variant of \TEL{} that allows both coping with finite traces and arbitrary combinations of past and future temporal operators, as those used in Linear Temporal Logic.


==> outline.tex <==
\makeatletter

%%% MALIPIVO's PDF SPECIAL TO CHANGE FONT OUTLINE THICKNESS/COLOR
% https://tex.stackexchange.com/questions/18472/tikz-halo-around-text/169549#169549
\input pdf-trans
\newbox\qbox
\def\usecolor#1{\csname\string\color@#1\endcsname\space}
\newcommand\bordercolor[1]{\colsplit{1}{#1}}
\newcommand\fillcolor[1]{\colsplit{0}{#1}}
\newcommand\outline[1]{\leavevmode%
  \def\maltext{#1}%
  \setbox\qbox=\hbox{\maltext}%
  \boxgs{Q q 2 Tr \thickness\space w \fillcol\space \bordercol\space}{}%
  \copy\qbox%
}
\makeatother
\newcommand\colsplit[2]{\colorlet{tmpcolor}{#2}\edef\tmp{\usecolor{tmpcolor}}%
  \def\tmpB{}\expandafter\colsplithelp\tmp\relax%
  \ifnum0=#1\relax\edef\fillcol{\tmpB}\else\edef\bordercol{\tmpC}\fi}
\def\colsplithelp#1#2 #3\relax{%
  \edef\tmpB{\tmpB#1#2 }%
  \ifnum `#1>`9\relax\def\tmpC{#3}\else\colsplithelp#3\relax\fi
}
\bordercolor{black}
\fillcolor{white}
\def\thickness{.3}

\renewcommand{\until}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{U}}$}}}}}
\renewcommand{\release}{\ensuremath{\mathbin{\mbox{\outline{$\bm{\mathsf{R}}$}}}}}
\renewcommand{\finally}{\ensuremath{\mbox{\outline{$\bm{\mathsf{F}}$}}}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

